Generalizations of Knotoids and Spatial Graphs

In 2010, Turaev introduced knotoids as a variation on knots that replaces the embedding of a circle with the embedding of a closed interval with two endpoints which here we call poles. We define generalized knotoids to allow arbitrarily many poles, intervals, and circles, each pole corresponding to any number of interval endpoints, including zero. This theory subsumes a variety of other related topological objects and introduces some particularly interesting new cases. We explore various analogs of knotoid invariants, including height, index polynomials, bracket polynomials and hyperbolicity. We further generalize to knotoidal graphs, which are a natural extension of spatial graphs that allow both poles and vertices.

==> sections/alexpoly.tex <==
\color{green} most likely scrap this for now until we have a more general/intuitive construction

The Alexander polynomial has proved to be a powerful invariant for knots and links. We review a few of the several constructions of the classical Alexander polynomial. Then, we extend the Alexander polynomial to planar staked links and further to staked multiknotoids using Gügümcü and Kauffman's Alexander polynomial for planar multiknotoids. 

\subsection{The Classical Alexander Polynomial}
To-Do: {\color{green} Describe the classical Alexander polynomial defined through Seifert surfaces and state sum w/ skein relation, note why important to be in $S^3$ for the following constructions}

\subsection{Alexander Polynomial for Planar Staked Links}
Recall from Example \ref{staked-links} that \emph{staked links} are generalized knotoids with diagrams appearing as classical link diagram with valency-zero poles placed in the regions of the link’s complement. We consider staked links with planar diagrams. 


Given an oriented staked link $L_s$ on a planar projection surface $\Sigma \times \{\frac{1}{2}\}$ in $\Sigma \times I$, we denote the set of its isolated poles as $\{p_1, …, p_n\}$ for $n \geq 1$, $p_i \neq p_j$ and the disk of radius sufficiently large to contain the link diagram and all its poles as $\mathcal{D} \subset \Sigma \times \{\frac{1}{2}\}$. To each of the poles $p_i$, we associate a line segment $\ell_i := p_i \times I$. Take open neighborhoods $\mathring{N}(\ell_i)$ of these line segments sufficiently small to ensure that this collection is also disjoint. The complement of this collection in $\mathcal{D} \times I$, $H_n^{L_s} := (\mathcal{D} \times I) \backslash \bigcup_i^n \mathring{N}(\ell_i)$ is now a handlebody of genus $n$ with a link embedded inside of it. 

For the purposes of defining an Alexander polynomial, we want to return from $H_n^{L_s}$ to $\Sigma \times I \subset S^3$ (We discuss in \ref{} the difficulty in defining an Alexander polynomial in a higher genus surface instead of $S^3$) To do this, we choose a point $q$ in $\Sigma \backslash \mathcal{D}$, dissolve each handle of $H_n^{L_s}$, then add a corresponding meridional unknot component encircling the removed handle and connecting the point $q$ to $p_i$ in $(\mathcal{D} \times I) \backslash H_n^{L_s}$ as in Figure \ref{}. We also dissolve handles with no link strands contained in them.\\
Performing this operation for each handle yields a link $\Tilde{L_s}$ in $S^3$ with $n$ added unknot components. It is straightforward to see that any choice of the point $q$ in $\Sigma \backslash \mathcal{D}$ yields equivalent links in $S^3$.\\

{\color{green} Picture of adding meridional components}\\

\begin{definition}
We define the Alexander polynomial of the oriented planar staked link $L_s$ as the Alexander polynomial of the oriented link $\Tilde{L_s}$,
$\Delta(L_s) = \Delta(\Tilde{L_s}) =$ det$(V - tV^t)$ 
\end{definition}

with $V$ the Seifert matrix with entries the pairwise linking numbers of first homology generating loops of the Seifert surface of $L$, and $t$ the polynomial variable as in the conventional Alexander polynomial definition in $S^3$. 


\begin{remark} 
Since we are on a planar projection surface, we can define the \textit{exterior region} of the staked link diagram to be the ``infinite'' connected component of the link complement, possibly including isolated poles. \\
Staked links $L_s$ with pole(s) in the exterior region of the knot diagram yields a handlebody with handle(s) containing no link strands after removing pole neighborhoods. These handles, which would otherwise result in an Alexander polynomial of 0 (as the corresponding link $\Tilde{L_s}$ in $S^3$ is split), get dissolved in the final $H_n^{L_s}$. Thus, adding poles in the exterior region of a planar staked link diagram does not alter the Alexander polynomial in our construction. 
\end{remark}

\begin{remark}
    When finding the Alexnder polynomial through taking the first homology of the infinite cyclic cover the link complement as in (Rolfsen) \ref{}, we rely on the trivial first homology of $S^3$ to ensure that all homology generators come from the link rather than the ambient space. Performing this in a handlebody rather than $S^3$ results in first homology generators from the ambient space and it is not clear how these generators should interact with the loops that come from the link itself, in particular, how these ambient space generators should be treated under the Laurent polynomial module. 
\end{remark}

\subsection{Alexander Polynomial for Multiknotoids}

Using this method of adding meridional unknot components to map a link in the handlebody to $S^3$ along with work of Gügümcü and Kauffman in \ref{}, we define an Alexander polynomial for planar \emph{staked multiknotoids}, generalized knotoids whose diagrams appear as a multiknotoid diagram with valency-zero poles placed in the regions of the multiknotoid’s complement.

We review the construction of the Alexander polynomial for knotoids given in \ref{} which directly extends to multiknotoids.\\

A \emph{Morse multiknotoid diagram} is a planar multiknotoid diagram arranged so that every horizontal line in the plane meets the diagram in at most one minimum, maximum, or crossing point defined with respect to the vertical direction of the plane. \\

{\color{green} Picture + describe parts of Morse knotoid diagram – crossings, cups, caps}\\

A Morse multiknotoid diagram is \emph{standard} if the tangent vectors at its endpoints of the knotoid component both point upward or downward. 

\begin{proposition} \ref{} 
Two oriented planar multiknotoid diagrams are equivalent if and only if their standard Morse diagrams are equivalent. 
\end{proposition}
\begin{proof}
    Gügümcü and Kauffman prove this for knotoids using \ref{} which gives the result for $(n,m)$-tangles of which multiknotoids are also examples, so this proof extends as desired.  
\end{proof}

Thus, to each oriented planar multiknotoid we can assign a unique oriented standard Morse multiknotoid diagram. 

The Alexander polynomial for oriented Morse multiknotoids is defined by a state sum model of the form $\Sigma_{\sigma} \langle K|_{\sigma} \rangle \delta^{\sigma}$ with $\delta$ the value of the state components, where a state is a configuration of crossing smoothings in the diagram. 
For multiknotoids, each state contains exactly one open-ended segment component and possibly many circular components. 

The values of the state components are given as in Figure \ref{}

Strands at the smoothing site in each state are given a label from the set \{+1, -1\}. 

Components of a state are also assigned a \emph{rotation number} defined as half of the sum of the signs on the maxima and minima in the diagram with rightward-oriented maxima and leftward-oriented minima having a sign of -1 and leftward-oriented maxima and rightward-oriented minima having a sign of 1. According to Theorem 1 of \ref{}, the rotation number is a Morse isotopy invariant.\\

{\color{green} Picture}\\

The state sum of an oriented Morse knotoid $K$ is defined as 
\begin{equation}
\Tilde{\Delta}_K = \Sigma_{\sigma} \langle K|_{\sigma} \rangle i^{||\sigma ||} 
\end{equation}

$\langle K|_{\sigma} \rangle$ denotes the product $\prod_i c_i$ where $i$ runs through all the resolved crossings in $\sigma$ where $c_i$ are the coefficients of the appropriately labelled crossing smoothing as given in Figure \ref{} \\ 

{\color{green} add figure for crossing smoothing coefficients}

These coefficients $c_i$ are derived from matrices defined in Section ??? of \ref{} that represent Morse knotoid components. \\
The matrices {\color{green} add matrices below} given for the construction of the Alexander polynomial in Section 5.2 satisfies certain equivalence conditions for Morse knotoids, namely the Yang-Baxter equation. {\color{green} I might fix up the wording here once I add in diagrams + their captions}

$||\sigma||$ denotes the sum of the labels of the loop components and the segment component in the state $\sigma$ multiplied by the rotation number of the components. 

\begin{proposition} \ref{}
The matrix given by state sum $\Tilde{\Delta}$ is a Morse isotopy invariant
\end{proposition}

Morse isotopy invariance is sufficient for invariance under knotoid Reidemeister II and III moves. Invariance under knotoid Reidemeister I moves requires a normalization factor $iq^{-rot(K)}$. 

\begin{definition}
The \emph{Alexander Polynomial for oriented planar multiknotoids} $\Delta_{MK}= \frac{1}{2} tr(iq^{-rot(MK)} \Tilde{\Delta}_{MK})$ 
\end{definition}

\begin{corollary}
The Alexander Polynomial for oriented planar multiknotoids $\Delta_{MK}= \frac{1}{2} tr(iq^{-rot(MK)} \Tilde{\Delta}_{MK})$ is an invariant of planar knotoids. 
\end{corollary}

\begin{remark}
There exist multiknotoid diagrams that admit no unknotting sequence obstructing the skein relation recursive computation for the Alexander polynomial as is described for classical links. Gügümcü and Kauffman's definition avoids this obstruction. See Figure \ref{}
\end{remark}

{\color{green} Picture of irreducible state components in unknotting recursion}\\

We use the correspondence described between staked diagrams and link diagrams in handlebodies to extend Gügümcü and Kauffman’s Alexander polynomial for multiknotoids to staked multiknotoids. 

In particular, for each pole of the $n$ poles of a multiknotoid diagram, we perform the operation of removing a stake neighborhood of the pole to yield a handlebody containing a multiknotoid diagram $H_n^{MK}$.

To convert $H_n^{MK}$ into a multiknotoid in $S^3$, we add meridional unknot components and dissolve appropriate handles as described previously and depicted in Figure \ref{} resulting in a multiknotoid with $n$ added unknot components in $S^3$, $\Tilde{MK_s}$. \\

{\color{green} Picture of staked multiknotoid diagram to multiknotoid in $S^3$}\\

\begin{definition}
We define the Alexander polynomial of the staked multiknotoid to be the Alexander polynomial for the multiknotoid $\Tilde{MK_s}$: \\$MK_s, \Delta(MK_s)  = \Delta(\Tilde{MK_s}) = \frac{1}{2} tr(iq^{-rot(MK)} \Tilde{\Delta}_{MK})$ 
\end{definition}

\begin{remark}
The Alexander polynomial for staked multiknotoids defined from the state-sum reduces to the Alexander polynomial we defined for staked knots.
\end{remark}


